Look, Radiate, and Learn: Self-Supervised Localisation via Radio-Visual Correspondence

Next generation cellular networks will implement radio sensing functions alongside customary communications, thereby enabling unprecedented worldwide sensing coverage outdoors. Deep learning has revolutionised computer vision but has had limited application to radio perception tasks, in part due to lack of systematic datasets and benchmarks dedicated to the study of the performance and promise of radio sensing. To address this gap, we present MaxRay: a synthetic radio-visual dataset and benchmark that facilitate precise target localisation in radio. We further propose to learn to localise targets in radio without supervision by extracting self-coordinates from radio-visual correspondence. We use such self-supervised coordinates to train a radio localiser network. We characterise our performance against a number of state-of-the-art baselines. Our results indicate that accurate radio target localisation can be automatically learned from paired radio-visual data without labels, which is important for empirical data. This opens the door for vast data scalability and may prove key to realising the promise of robust radio sensing atop a unified communication-perception cellular infrastructure. Dataset will be hosted on IEEE DataPort.

==> src_appen/acronyms.tex <==
\begin{multicols}{2}
\begin{acronym}[WSSUS]
    
    
    
    
    \acro{3GPP}{3rd Generation Partnership Project}
    \acro{5G}{fifth-generation}
    \acro{ADC}{analog to digital converter}
    \acro{AFE}{analog front end}
    \acro{AGC}{automatic gain control}
    \acro{AGV}{automated guided vehicle}
    \acro{AMP}{approximate message passing}
    \acro{API}{Application Programming Interface}
    \acro{AWGN}{additive white Gaussian noise}
    \acro{AutoML}{automatic-machine-learning}
    \acro{BER}{bit error rate}
    \acro{BB}{baseband}
    \acro{bpcu}{bits per channel use}
    \acro{BP}{belief propagation}
    \acro{BPSK}{binary phase shift keying}
    \acro{BS}{base station}

    \acro{CFAR}{Constant-False-Alarm-Rate}
	\acro{CL}{Constrastive Loss}
	\acro{MCL}{Masked contrastive Loss}
    \acro{CB}{codebook}
    \acro{CDF}{cumulative distribution function}
    \acro{CFO}{carrier frequency offset}
    \acro{CoSaMP}{compressive sampling matching pursuit}
    \acro{CP}{cyclic prefix}
    \acro{CS}{compressive sensing} 
    \acro{CSI}{channel state information}
    \acro{CNN}{convolutional neural network}

    \acro{DA}{domain adaptation}
    \acro{DBSCAN}{Density-Based Spatial Clustering of Applications with Noise}
    \acro{DAC}{digital-analog-converter}
    \acro{DC}{direct current}
    \acro{DE}{distance error}
    \acro{DeepL}{deep-learning}
    \acro{DoF}{degree-of-freedom}
    \acro{DFT}{discrete Fourier transformation}
    \acro{DL}{deep learning}
    \acro{DS}{delay spread}
    \acro{DSP}{digital signal processing}

    \acro{ECC}{error-correcting code}
    \acro{ENoB}{effective number of bits}
    \acro{ERP}{effective radiated power}
    \acro{EVM}{error vector magnitude}
    \acro{EVD}{eigenvector decomposition}
    \acro{FB}{feedback}
    \acro{FC}{fully connected}
    \acro{FDD}{frequency division duplexing}
    \acro{FDM}{frequency division multiplexing}
    \acro{FIR}{finite impulse response}
    \acro{FFT}{fast fourier transform}
    \acro{FT}{fine tuning}
    \acro{FPGA}{field programmable gate array}
    \acro{GAN}{Generative adversarial network}
    \acro{GPIO}{general-purpose input/output}
    \acro{GPS}{global positioning system}
    \acro{GPSDO}{GPS disciplined oscillator}
    \acro{GPU}{graphical processing unit}
    \acro{HDF}{Hierarchical Data Format}
    \acro{HDD}{hard decision decoding}
    \acro{IC}{integrated circuit}
    \acro{ICI}{inter-carrier-interference}
    \acro{ISAC}{Integrated Sensing And Communication}
    \acro{I2C}{Inter-Integrated Circuit}
    \acro{ICSP}{in-circuit serial programming}
    \acro{IF}{intermediate frequency}
    \acro{i.i.d.}{independent and identically distributed}
    \acro{IIR}{infinite impulse response}
    \acro{IMU}{inertial measurement unit}
    \acro{IoT}{Internet of Things}
    \acro{IPS}{indoor positioning system}
    \acro{IR}{infrared}
    \acro{JSDM}{Joint Spatial Division and Multiplexing}
    \acro{LIDAR}{Light Detection And Ranging}
    \acro{LLR}{log-likelihood ratio}
    \acro{LP}{leakage precoder}
    \acro{LMMSE}{Linear Minimum Mean Square Error}
    \acro{LO}{local oscillator}
    \acro{LoS}{line of sight}
    \acro{LiDaR}{Light Detection and Ranging}
    \acro{LS}{least squares}
    \acro{LSTM}{long-term short-term memory}
    \acro{LTE}{Long Term Evolution}
    \acro{LTI}{linear time invariant}
    \acro{LTV}{linear time variant}
  
    \acro{MAP}{maximum a posteriori}
    \acro{MDE}{mean distance error}
    \acro{MDA}{mean distance accuracy}
    \acro{MEMS}{Micro-Electro-Mechanical Systems}
    \acro{MIMO}{multiple input multiple output}
    \acro{MISO}{multiple input single output}
    \acro{ML}{maximum likelihood}
    \acro{MLD}{maximum likelihood decoding}
    \acro{mMIMO}{massive multiple input multiple output}
    \acro{MMSE}{minimum mean square error}
    \acro{M-MMSE}{multi-cell minimum mean square error}
    \acro{MR}{maximum ratio}
    \acro{MRC}{maximum ratio combining}
    \acro{MRP}{maximum ratio precoding}
    \acro{MRT}{maximum ratio transmission}
    \acro{MSE}{mean squared error}
    \acro{MQTT}{Message Queuing Telemetry Transport}
    \acro{MU}{multi-user}
    \acro{MUSIC}{Multiple Signal Classification}
    \acro{NF}{noise figure}
    \acro{NN}{Neural Network}
    \acro{NNI}{Neural Network Intelligence}
    \acro{NLoS}{non-line of sight}
    \acro{NND}{neural network decoding}
    \acro{NTP}{Network Time Protocol}
    \acro{NMSE}{normalized mean squared error}
    \acro{NU}{not-used}
    \acro{OFDM}{orthogonal frequency division multiplex}
    \acro{OMP}{orthogonal matching pursuit}
    \acro{OPS}{outdoor positioning system}
    \acro{OT}{optimal transport}
    \acro{PB}{passband}
    \acro{PCB}{printed circuit board}
    \acro{PDR}{pedestrian dead reckoning}
    \acro{PDF}{probability density function}
    \acro{PDP}{power-delay-profile}
    \acro{PLL}{phase-locked-loop}
    \acro{PO}{phase-only}
    \acro{PPS}{pulse per second}
    \acro{QPSK}{quadrature phase shift keying}
    \acro{QuaDRIGa}{Quasi Deterministic Radio Channel Generator}

    \acro{RADAR}{Radio Detection And Ranging}
    \acro{ReLU}{rectified linear unit}
    \acro{RF}{radio frequency}
    \acro{RMS-DS}{Root Mean Square - Delay Spread}
    \acro{RNN}{recurrent neuronal network}
    \acro{RSSI}{received signal strength indicator}
    \acro{R-ZF}{regularized zero-forcing}
    \acro{SDD}{soft decision decoding}
    \acro{SDR}{software defined radio}
    \acro{SE}{spectral efficiency}
    \acro{SFO}{sampling frequency offset}
    \acro{STO}{sampling time offset}
    \acro{SLAM}{Simultaneous Localization and Mapping}
    \acro{SGD}{stochastic gradient descent}
    \acro{SISO}{single input single output}
    \acro{SINR}{signal-to-interference-and-noise-ratio}
    \acro{SIR}{signal-to-interference-ratio}
    \acro{SLNR}{signal-to-leakage-and-noise ratio}
    \acro{SNR}{signal-to-noise-ratio}
    \acro{SP}{subspace}
    \acro{SQR}{signal-to-quantization-noise-ratio}
    \acro{SQNR}{signal-to-quantization-noise-ratio}
    \acro{SVD}{singular value decomposition}
    \acro{SU}{single-user}
    \acro{TDD}{time division duplexing}
    \acro{TRIPS}{time-reversal IPS}
    \acro{UE}{user equipment}
    \acro{UL}{uplink}
    \acro{ULA}{uniform line array}
    \acro{URLLC}{ultra-reliable low-latency communication}
    \acro{US}{uncorrelated scattering}
    \acro{USRP}{universal software radio peripheral}
    \acro{UWB}{ultra-wideband}
    \acro{WiFi}{Wireless Fidelity}
    \acro{WSS}{wide sense stationary}
    \acro{WSSUS}{wide sense stationary uncorrelated scattering}

    \acro{ZF}{zero forcing}
\end{acronym}
\end{multicols}


==> src_main/datasheet.tex <==
\onecolumn
\section{Datasheet} \label{sec:datasheet}

We document in Tab.~\ref{tab:dataset_datasheet} various aspects of our radio-visual dataset according to the specifications stipulated in~\cite{gebru2021datasheets}.

\begin{scriptsize}
\begin{longtable}{QA}
\caption{Dataset datasheet}
\label{tab:dataset_datasheet}

\endfirsthead

\toprule
\multicolumn{2}{c}{Cont. Tab.~\ref{tab:dataset_datasheet}}\\
\endhead

\cmidrule(lr){1-2}
\multicolumn{2}{c}{End Tab.~\ref{tab:dataset_datasheet}}\\
\bottomrule
\endlastfoot

\toprule
\multicolumn{2}{c}{Motivation}   \\
\cmidrule(lr){1-2}
For what purpose was the dataset created? 
& To facilitate radio-visual SSL research for 6G sensing. \\
Who created the dataset and on behalf of which entity? 
& Bell Labs Core Research (BLCR) on behalf of Nokia. \\
Who funded the creation of the dataset? 
& Nokia. \\
\cmidrule(lr){1-2}
\multicolumn{2}{c}{Composition}   \\
\cmidrule(lr){1-2}
What do the instances that comprise the dataset represent? 
& heatmap-image pairs sampled from a parking lot scenario. \\
How many instances are there in total? 
& 30,000 labelled for parking lot. \\ % 10,000 labeled for suburban and 10,000 labeled for canyon \\
Does the dataset contain all possible instances or is it a sample of instances from a larger set?  
& All. \\
What data does each instance consist of?  
& Radio heatmaps are range-azimuth description of the environment and RGB images are their visual pairs. \\
Is there a label or target associated with each instance?  
% & For labelled set, object groundtruth coordinates for radio and scenario label.  \\
& Object groundtruth coordinates for radio and bounding boxes for vision. \\
Is any information missing from individual instances? 
& No. \\
Are relationships between individual instances made explicit?  
& Correspondence between each radio-visual pair. \\
Are there recommended data splits? 
& 80:20 train-validation split for downstream regression. \\
Are there any errors, sources of noise, or redundancies in the dataset? 
& Not at the data instance level; It is a synthetic dataset. At the radio signal level, high-fidelity propagation modelling captures non-trivial sources of noise such as clutter and fading. \\
Is the dataset self-contained, or does it link to or otherwise rely on external resources? 
& Self-contained. \\
Does the dataset contain data that might be considered confidential? 
& No. \\
Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?  
& No. \\
Does the dataset identify any subpopulations?  
& No. \\
Is it possible to identify individuals, either directly or indirectly from the dataset?  
& No. \\
Does the dataset contain data that might be considered sensitive in any way?  
& No. \\
\cmidrule(lr){1-2}
\multicolumn{2}{c}{Collection Process}   \\
\cmidrule(lr){1-2}
How was the data associated with each instance acquired?  
& Synthesised using CAD tools. \\
What mechanisms or procedures were used to collect the data?  
& Ray-tracing for radio and rendering for vision. \\
If the dataset is a sample from a larger set, what was the sampling strategy? 
& N/A. \\
Who was involved in the data collection process and how were they compensated?  
& Nokia employees under full-time employment. \\
Over what timeframe was the data collected?  
& Data generation took several months of in-house development effort. \\
Were any ethical review processes conducted?  
& N/A. \\
Did you collect the data from the individuals in question directly, or obtain it via third parties or other sources?  
& N/A. \\
Were the individuals in question notified about the data collection?  
& N/A. \\
Did the individuals in question consent to the collection and use of their data?  
& N/A. \\
If consent was obtained, were the consenting individuals provided with a mechanism to revoke their consent in the future or for certain uses?  
& N/A. \\
Has an analysis of the potential impact of the dataset and its use on data subjects been conducted?  
& N/A. \\
\cmidrule(lr){1-2}
\multicolumn{2}{c}{Preprocessing/cleaning/labeling}   \\
\cmidrule(lr){1-2}
Was any preprocessing/cleaning/labeling of the data done?  
& No. \\
Was the ``raw'' data saved in addition to the preprocessed/cleaned/labeled data?  
& N/A. \\
Is the software that was used to preprocess/clean/label the data available?  
& N/A. \\
\cmidrule(lr){1-2}
\multicolumn{2}{c}{Uses}   \\
\cmidrule(lr){1-2}
Has the dataset been used for any tasks already? 
& Mainly radio-visual SSL research disclosed in this paper. \\
Is there a repository that links to any or all papers or systems that use the dataset?  
& N/A. \\
What (other) tasks could the dataset be used for?  
% & This is a 1st radio-visual SSL work, and future research would build on our ideas and/or come up with alternative approaches, e.g., non-contrastive SSL. \\
& This is a 1st radio-visual SSL work, and future research would build on our ideas and/or investigate alternative approaches, e.g., for more discriminative radio signals obtained from finer angular resolutions. \\
Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?  
& No. \\
Are there tasks for which the dataset should not be used?  
& N/A. \\
\cmidrule(lr){1-2}
\multicolumn{2}{c}{Distribution}   \\
\cmidrule(lr){1-2}
Will the dataset be distributed to third parties outside of the entity on behalf of which the dataset was created?  
& Yes. \\
How will the dataset will be distributed?  
& Hosted on a public website. \\
When will the dataset be distributed?  
& 2023. \\
Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?  
& Yes. \\
Have any third parties imposed IP-based or other restrictions on the data associated with the instances?  
& No. \\
Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?  
& No. \\
\cmidrule(lr){1-2}
\multicolumn{2}{c}{Maintenance}   \\
\cmidrule(lr){1-2}
Who will be supporting/hosting/maintaining the dataset?  
& Nokia Bell Labs. \\
How can the owner/curator/manager of the dataset be contacted?  
& Email. \\
Is there an erratum?  
& No. \\
Will the dataset be updated?  
& Yes. \\
If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances?  
& N/A. \\
Will older versions of the dataset continue to be supported/hosted/maintained?  
& Yes. \\
If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?  
& We will provide reference Blender files which can be modified to model different environments.
Our radio raytracing is however proprietary and cannot be released.
To work around this, users could licence equivalent commercial radio raytracers in order to generate paired radio heatmaps from Blender's 3D models. \\
\end{longtable}
\end{scriptsize}
\twocolumn



==> src_main/deepsense.tex <==
% \vspace{-0.25cm}
\newpage
\section{Preliminary Empirical Results} \label{sec:empirical_results}

In this section we apply our radio-visual SSL algorithm on DeepSense.
DeepSense is a recent empirical dataset curated for 6G use cases, including sensing~\cite{DeepSense}.
The preliminary results we present herein are intended as a further validation of our SSL algorithm on a snippet of real-world data.
We begin by comparing DeepSense to~\dataset.


\begin{table}[H]
    \vspace{-0.25cm}
  \caption{Comparison between~\dataset~and DeepSense. DeepSense requires preprocessing for integration into our radio-visual SSL algorithm.}
  \label{tab:maxray_vs_deepsense}
  \scriptsize
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{lEEE}
    \toprule
    Entry     & MaxRay                                       & DeepSense                         & Preprocessing  \\
    \cmidrule(lr){1-4}
    Camera    & 30 FPS @ 640$\times$480 pixels               & 30 FPS @ 960$\times$540 pixels    & Linear downscaling to 640$\times$480 \\
    Radio     & OFDM Radar @ 800MHz BW, dense 16$\times$16 antenna array   & FMCW Radar @ 750MHz BW, sparse 4$\times$2 antenna array & Radar range filtered to 5-25m, and periodogram upsampled \\
    Radio groundtruth  & Perfect high-fidelity ray tracing   & RTK GPS as pseudo groundtruth     & Converting GPS to pseudo range and azimuth \\
    Vision groundtruth & Perfect target bounding box         & Yolo v5 target bounding box & None                                          \\
    Scenario      & See Sec.~\ref{sec:dataset} & Multiple, see~\cite{DeepSense}      & None \\
    \bottomrule
  \end{tabular}}
\end{table}
\vspace{-0.25cm}

Tab.~\ref{tab:maxray_vs_deepsense} illustrates the differences between~\dataset and DeepSense.
\dataset~uses OFDM radar that integrates within communication networks as treated in Appendix~\ref{sec:appendix_ofdm_radar}.
OFDM radar is higher-power and higher-fidelity compared to DeepSense's FMCW radar.
FMCW radar is essentially an analogue technology that dates back to the 1st half of the 20th century~\cite{Charvat14_SmallAndShortRangeRadarSystems}.
We also highlight that in~\dataset, we model and control the environment to generate perfect groundtruth.

\subsection{DeepSense pseudo label construction}

We construct two pseudo labels for DeepSense's vision and radio entries. 
For vision, we forward pass DeepSense's camera images through a Yolov5 model to obtain bounding boxes.
We verify through manual inspection that this procedure detects target cars.
For radio, we convert the highly accurate RTK GPS measurements (i.e., trilaterations) into local coordinates.
The radio basestation has longitudinal and latitudinal coordinates. 
Using~\cite{van_BidirectionalUTM}, we convert these coordinates into a Cartesian frame.
This process can give rise to bias as it ignores the heights of the basestation and cars. 
We, therefore, perform one-off calibration to minimise range and angle errors.

\subsection{Preliminary experiment}

\noindent \textbf{Data \& setup.}
DeepSense has a phased release plan. 
At the time of writing, only a small portion of the full dataset is available.
Of the available subset, Scenario 9\footnote{\url{https://deepsense6g.net/scenario-9/}} is the closest useful portion that can be used to evaluate empirically radio-visual SSL.
Scenario 9 contains cars that drive on a street from left to right for 5 hours.
A camera and a radio basestation that are mounted on tripods record measurements. 
The vision entries have good lighting conditions. 
Scenario 9 has currently a total of 5200 data points, of which only 4219 contain fully visible cars.
We train the SCL variant of our radio-visual SSL algorithm on these 4219 data points.
We use the same implementation details from Sec.~\ref{sec:implement_details}.

\begin{wrapfigure}[24]{r}{0.40\textwidth}
  \begin{center}
    \vspace{-0.50cm}
    \includegraphics[width=0.3\textwidth]{./img/range_train_dists_scl_deepsense6g}
  \end{center}
  \caption{Preliminary results for DeepSense Scenario 9. SCL self-labels and GPS pseudo groundtruth overlaid.}
  \label{fig:deepsense-results}
  \vspace{-0.25cm}
\end{wrapfigure}
\noindent \textbf{Results.}
We derive SCL self-labels using cross-modal attention maximisation as detailed in Sec.~\ref{sec:representation_learning} (cf., Eqs.~\ref{eq:2d_attention}~\&~\ref{eq:max_2d_attention}).
Fig.~\ref{fig:deepsense-results} overlays range self-labels and GPS range pseudo labels. 
We can readily see that with as little as 4k data points, cross-modal attention from the SCL backbone is able to learn to estimate range. 
Note that the edges of the two distributions deviate more. 
This is because the fixed mounting of the GPS unit does not sample car movements the way the radar does. 
Nonetheless, this crude experiment demonstrates that our radio-visual SSL algorithm is readily applicable to empirical data.


